Break the Chain: Large Language Models Can be Shortcut Reasoners

Recent advancements in Chain-of-Thought (CoT) reasoning utilize complex modules but are hampered by high token consumption, limited applicability, and challenges in reproducibility. This paper conducts a critical evaluation of CoT prompting, extending beyond arithmetic to include complex logical and commonsense reasoning tasks, areas where standard CoT methods fall short. We propose the integration of human-like heuristics and shortcuts into language models (LMs) through "break the chain" strategies. These strategies disrupt traditional CoT processes using controlled variables to assess their efficacy. Additionally, we develop innovative zero-shot prompting strategies that encourage the use of shortcuts, enabling LMs to quickly exploit reasoning clues and bypass detailed procedural steps. Our comprehensive experiments across various LMs, both commercial and open-source, reveal that LMs maintain effective performance with "break the chain" strategies. We also introduce ShortcutQA, a dataset specifically designed to evaluate reasoning through shortcuts, compiled from competitive tests optimized for heuristic reasoning tasks such as forward/backward reasoning and simplification. Our analysis confirms that ShortcutQA not only poses a robust challenge to LMs but also serves as an essential benchmark for enhancing reasoning efficiency in AI.

==> subtexs/ablation.tex <==
\subsection{Ablation Studies}
(don't know how to deal with this part. maybe move the experiments of model size in discussion)
Ablation studies were designed to isolate the specific components of the ``break the chain'' methodology that contribute most significantly to observed performance changes. By systematically removing or altering elements of our prompting strategy, we aimed to uncover the underlying mechanisms that facilitate or hinder effective reasoning.

Each ablation study focused on one aspect of the ``break the chain'' prompt, such as the removal of intermediate reasoning steps, changes in prompt length, or variations in the clarity of instructions. The performance impact of these modifications was measured against standard CoT and ``break the chain'' outcomes.

Results from our ablation studies provide insights into:
The critical components of effective ``break the chain'' prompts.
The extent to which instruction-tuned models rely on the structure and content of prompts.
Strategies for optimizing prompt design to leverage the full potential of both instruction-tuned and base LLMs.

Our comparative analysis and ablation studies shed light on the intricate relationship between LLMs' reasoning capabilities and the structure of prompts. Our findings suggest a more nuanced interaction, indicating areas for future exploration in model training and prompt engineering.


==> subtexs/case_study.tex <==

% \begin{figure*}[ht]
%   \centering
%   \begin{subfigure}{\linewidth} % subfigure占据整个列宽
%     \includegraphics[width=\textwidth]{figures/graph/syllogism_zero_CoT.png}
%     \caption{Using zero-shot CoT prompt: Let's think step by step}
%     \label{fig:sub1}
%   \end{subfigure}% 别忘了百分号来避免不必要的空格
  
%   \vspace{1em} % 提供两个子图之间的垂直空间
  
%   \begin{subfigure}{\linewidth} % subfigure再次占据整个列宽
%     \includegraphics[width=\textwidth]{figures/graph/syllogism_promptQC.png}
%     \caption{Using "Break the Chain" promptQC: Let's quickly conclude the answer without showing step-by-step reasoning.}
%     \label{fig:sub2}
%   \end{subfigure}
  
%   \caption{Data example of Syllogism Problems from the ShortcutQA dataset, along with an illustration of the basic process for generating and extracting answers.}
%   \label{fig:syllogism_data}
% \end{figure*}


==> tables/data_bak.tex <==
\begin{center}
\begin{table*}[h!]
\begin{tabular}{ c c c c c c} 
 \hline
 Dataset & Answer Format(*1) & \# of samples & Avg \# words(*2) & Data filename & License \\ 
 \hline
 SingleEq & N & 508 & 27.4 & questions.json & No License \\ 
 AddSub & N & 395 & 31.5 & AddSub.json & Unspecified\\ 
 MultiArith & N & 600 & 31.8 & MultiArith.json & Unspecified\\
 GSM8K & N & 1319 & 46.9 & test.jsonl & MIT License\\
 AQUA-RAT & C & 254 & 51.9 & test.jsonl & Apache-2.0\\
 SVAMP & N & 1000 & 31.8 & SVAMP.json & MIT License\\
 CommonsenseQA & C & 1221 & 27.8 & dev\_rand\_split.jsonl & Unspecified\\
 StrategyQA & Y & 2290 & 9.6 & task.json & Apache-2.0\\
 Date Understanding & C & 369 & 35.0 & task.json & Apache-2.0\\
 Shuffled Obejects & C & 750 & 91.1 & three\_objects/task.json & Apache-2.0\\
 LogiQA & C & &  & test.txt \& zh\_test.txt &\\
 ReClor & C & 500 &  & val.json &\\
 \hline
\end{tabular}
\caption{Dataset Description. Our experiments used publicly available datasets.
(*1) N : Number, C : Pick up one from multiple choices, Y : Answer Yes or No, (*2) Average number of words in questions.
}
\label{table:2}
\end{table*}
\end{center}

==> tables/few-shot.tex <==
\begin{table*}
\centering
\begin{tabularx}{0.82\textwidth}{c|l|c|c}
 \toprule
 Task & Dataset & Few-shot CoT & Few-shot "Break the Chain"\\ 
 \midrule
 \multirow{2}{*}{Arithmetic} & MultiArith & 99.00 & 98.33 \\ 
 & GSM8K & 74.60  & 74.22  \\ 
 \midrule
 \multirow{2}{*}{Commonsense} & CommonsenseQA & 74.94 & 75.18 \\ 
 & StrategyQA & 69.13  & 68.60  \\ 
 \midrule
 Logic & LogiQA & 35.94  & 33.95  \\
 \bottomrule
\end{tabularx}
\caption{ChatGPT performance on Few-Shot CoT and Few-Shot "breaking
the chain". All results are in \% accuracy.}
\label{table:few_shot_res}
\end{table*}
